VOICE: Variance of Induced Contrastive Explanations to quantify Uncertainty in Neural Network Interpretability

In this paper, we visualize and quantify the predictive uncertainty of gradient-based post hoc visual explanations for neural networks. Predictive uncertainty refers to the variability in the network predictions under perturbations to the input. Visual post hoc explainability techniques highlight features within an image to justify a network's prediction. We theoretically show that existing evaluation strategies of visual explanatory techniques partially reduce the predictive uncertainty of neural networks. This analysis allows us to construct a plug in approach to visualize and quantify the remaining predictive uncertainty of any gradient-based explanatory technique. We show that every image, network, prediction, and explanatory technique has a unique uncertainty. The proposed uncertainty visualization and quantification yields two key observations. Firstly, oftentimes under incorrect predictions, explanatory techniques are uncertain about the same features that they are attributing the predictions to, thereby reducing the trustworthiness of the explanation. Secondly, objective metrics of an explanation's uncertainty, empirically behave similarly to epistemic uncertainty. We support these observations on two datasets, four explanatory techniques, and six neural network architectures. The code is available at https://github.com/olivesgatech/VOICE-Uncertainty.

==> Sections/7_Response2Reviewers.tex <==
\section*{Response to Reviewers}

\noindent We thank the Associate Editors, the Guest Editors, and the Reviewers for their feedback and comments. We have addressed each of the raised points in the following response. 

\noindent The Reviewer comments are in blue. Our response is in black. In the revised and reuploaded paper, the changes are highlighted. 

\subsection{Reviewer 1}
\textcolor{blue}{1. The proposed method focus on the visual explanation on object/instance level semantic. Is there any experiment about the visual explanation on higher or lower level? For example, on scene level or component level? The component means the compositional parts of the objects, such as the tier, wind screen, and light of a car.}

The proposed method uses existing explanatory techniques' frameworks to quantify $V(y|S_x)$. The uncertainty of any higher level task (scene classification and visual question answering among others) that allows backpropagating alternative labels $y$ can be quantified using VOICE. For lower level tasks like fine-grained object detection, $y$ can be a classification label (leading to similar results as in the paper), or a bounding box regressor coordinate. A recent work [1] explores GradCAM from the perspective of bounding box regression and backpropagating perturbations to the bounding box coordinates. Constructing VOICE with respect to bounding box may be an alternative avenue for compositional parts explanation and uncertainty. In regression uncertainty estimation, prediction intervals are commonly used and a potential future work is to tie VOICE to conformal prediction errors and uncertainty.

[1] Nogueira, Caio, Luís Fernandes, João ND Fernandes, and Jaime S. Cardoso. "Explaining Bounding Boxes in Deep Object Detectors Using Post Hoc Methods for Autonomous Driving Systems." Sensors 24, no. 2 (2024): 516.

\textcolor{blue}{2. Given the well calculated uncertainty, it is similiar with the cross-attention mechanism, if there is any possible that we can implement it or include it in the attention calculation? Any experiment about it?}

We thank the reviewer for this insight. We had not considered the proposed methodology from the perspective of cross-attention and currently have no experiments on it. However, cross attention between image patches of varying scales have multiple disagreements that can be quantified and reduced using the proposed method. We will certainly consider this experimental modality in the near future.  

\subsection{Reviewer 2}
\textcolor{blue}{1. There is a practical issue with the metrics. The obtained IoU (same for SNR) metric has varying ranges across different visualization methods and network architectures. For instance, the IoU of Guided Backprop is always far less than other methods. Then how can we determine/compare the uncertainties of different methods? How do we know how big the IoU indicates what level of uncertainty? Properly addressing these problems would improve the applicability of the proposed metrics.}

As the reviewer notes, both SNR and IoU metrics are unbounded and have varying ranges across different explanations. This is the case for general UQ literature and the commonly used negative log-likelihood metric is also unbounded. However, we agree with the reviewer regarding the applicability of the proposed metrics and add an additional Subsection~\ref{subsec:Compare} and Table~\ref{tab:Results_Compare} that extends the CIFAR-10C experiments to compare between explanations. The text and table are reproduced below for convenience.

\subsection*{Comparing explanatory techniques}
Table~\ref{tab:Results_All} provides IoU and SNR quantification of VOICE that validates the overlap and dispersion hypotheses. However, these results are insufficient to compare between explanations. For instance, Guided Backpropagation has the highest difference between correct and incorrect prediction IoU across all architectures, except Swin transformer. An incorrect conclusion from the preceding statement is that guided backpropagation is the best method (as compared against GradCAM, GradCAM++, and SmoothGrad) since it has less overlap between the explanation and its uncertainty. This is an incorrect conclusion since the values of IoU is not comparable between explanatory methodologies. On AlexNet, the IoU of Guided Backpropagation is $0.047$ while on the other explanations, IoU is around $0.5$. Visually, the low IoU value of Guided Backpropagation uncertainty manifests itself as mostly black regions in Fig.~\ref{fig:Explanations_Correct} with the uncertain regions highlighted within the red box to make them apparent.

Note that the variability in metric range is a common issue within uncertainty quantification literature. For instance, log-likelihood measure is unbounded and differs based on network, data, and predictions. Since there is no ground truth, uncertainty evaluation strategies utilize a set of samples rather than individual predictions for a pseudo-classification task. In~\cite{benkerttransitional}, the authors utilize their proposed uncertainty metric to classify between in-distribution and out-of-distribution data. Higher the classification accuracy, better the uncertainty metric. In~\cite{lee2023probing}, the authors use Area Under Accuracy Curve (AUAC) on CIFAR-10C dataset to showcase that their uncertainty metric is robust against increasing level of challenges. Ideally, AUAC must remain high, even when a network is presented with challenging data. We follow the same procedure as~\cite{lee2023probing} and provide the Area Under IoU and Area Under SNR Curves for each of the four explanations on three challenges used in Section~\ref{subsec:Quantitative_challenging}. From Fig.~\ref{fig:CIFAR-10C}, the IoU and SNR VOICE quantification must ideally be zero across increasing level of challenges. An explanation with an AUC closer to zero is a better explanation. We calculate the area under both IoU and SNR measures and present them in Table~\ref{tab:Results_Compare}. The best performing explanation for every challenge and metric is bolded. Note that on average, GradCAM has both IoU and SNR values closer to zero compared to the other explanations. Our proposed explanation overcomes the masking limitations in existing explanatory evaluation techniques to objectively quantify subjective explanations.

\input{Table/tab_Compare}

\textcolor{blue}{2. References 17, 18, and 30 are missing the author names. The paper "Patro, Badri N., et al. "U-cam: Visual explanation using uncertainty based class activation maps." Proceedings of the IEEE/CVF International Conference on Computer Vision. 2019." (DOI: 10.1109/ICCV.2019.00754) discusses relevant topics and thus should be cited.}

Regarding the missing author names: The bib package recommended by IEEE for manuscript preparation, IEEEtran.bst, has an option for "dashification" of repeated author names enabled by default. We have disabled it in the re-submission and the author names in 17, 18, and 30 are now visible. 

We thank the reviewer for pointing us at the relevant citation. We have studied and agree with the reviewer regarding U-CAM's relevance. We have cited and added it in the Related Works section. The text is reproduced below:

Uncertainty in explainability is less researched in literature. This is partly because the goal of explainability is \emph{post hoc}, i.e. explanatory techniques act after a decision is made. On the other hand, UQ deals with estimating and reducing uncertainty of the decision itself. The authors in~\cite{patro2019u} incorporate uncertainty estimation during the training process to improve visual explanations at inference for the task of visual question answering. In~\cite{chowdhury2023explaining}, causal metrics of necessity and sufficiency are used to evaluate the uncertainty of explanations in tabular data.


